Welfare and Profit Maximization with Production Costs

Combinatorial Auctions are a central problem in Algorithmic Mechanism Design: pricing and allocating goods to buyers with complex preferences in order to maximize some desired objective (e.g., social welfare, revenue, or profit). The problem has been well-studied in the case of limited supply (one copy of each item), and in the case of digital goods (the seller can produce additional copies at no cost). Yet in the case of resources---oil, labor, computing cycles, etc.---neither of these abstractions is just right: additional supplies of these resources can be found, but at increasing difficulty (marginal cost) as resources are depleted. In this work, we initiate the study of the algorithmic mechanism design problem of combinatorial pricing under increasing marginal cost. The goal is to sell these goods to buyers with unknown and arbitrary combinatorial valuation functions to maximize either the social welfare, or the seller's profit; specifically we focus on the setting of \emph{posted item prices} with buyers arriving online. We give algorithms that achieve {\em constant factor} approximations for a class of natural cost functions---linear, low-degree polynomial, logarithmic---and that give logarithmic approximations for more general increasing marginal cost functions (along with a necessary additive loss). We show that these bounds are essentially best possible for these settings.

==> intro.tex <==
\section{Introduction}
\label{sec:overview}

%%%% Talk in terms of pricing or combinatorial auctions?
%%
%%%% Pricing
%%
%% One of the most basic problems in algorithmic economics is that of
%% pricing: how to assign prices to goods or services in the presence of
%% buyers with complex, combinatorial preference functions in order to
%% maximize some desired objective (e.g., social welfare or revenue).
%%
%%%% Comb auctions
%%
Combinatorial Auctions are a central problem in Algorithmic
Mechanism Design: pricing and allocating goods to buyers with
complex preferences in order to maximize some desired objective
(e.g., social welfare, revenue, or profit).  This problem is
typically studied in one of two extreme cases -- the case of
\emph{limited supply} (one copy of each item) or the case of
\emph{unlimited supply} (the seller can produce additional copies at
no cost). For the case of limited supply, there are strong negative
results (see \cite{BNisan} and the references therein) unless one
makes additional assumptions on the buyers' valuations (e.g., 
submodularity~\citep{DNS06,lln06,Dob07,CHK09}). In contrast, for
unlimited supply, which is characteristic of digital goods,
maximizing social welfare is trivial by giving all the items away
for free, and for revenue maximization, good bounds can be achieved
for general buyers~\citep{BHK08,BBM08}. However, in the case of
resources---whether oil or computing cycles or food or
attention span---the unlimited-supply case is too optimistic and the
limited-supply case too pessimistic. More often than not, additional
sources can be found, but at higher cost.
%YM
Indeed, the classical market equilibrium in economic theory assumes
that as prices rise, supply increases while demand
decreases (giving a unique price which clears the market). 
%%The increasing supply implies that the cost of production 
Such a supply curve corresponds to a cost of obtaining goods that 
increases with the number of items desired.
%%produced.
%Indeed, much of
%traditional economic theory going back to Cournot competition
%assumes a concave economy with convex (cumulative) production costs
%of exactly this type~\citep{MWG95}.

In this work, we initiate the study of this setting where additional
resources can be found, but at \emph{increasing marginal cost},
%%, so that the algorithm ends up with a deficit while the optimal social
%%welfare or revenue is always non-negative making a non-trivial welfare
%%or revenue guarantee on part of the algorithm an `infeasible' proposition.}
for the algorithmic mechanism design problem of combinatorial pricing.\footnote{One could also study decreasing marginal costs, though we point out that modeling decreasing marginal costs in a non-Bayesian adversarial setting poses difficulties.   For example, there are situations where any algorithm can make positive profit only by initially going into deficit, at which point the adversary could send in no more buyers.} 
That is, a seller has $n$ goods, and for each good $i$ there is a non-decreasing marginal cost function $c_i()$, capturing the fact that additional units of this good can be obtained, but at an increasing difficulty to the seller per unit.
%%producing or acquiring each additional unit costs no less than that of the previous units.
%%Increasing marginal costs capture the production costs of scarce resources, 
%%or any market where increased demand causes the cost per item to rise.
%%such as petroleum, where every additional gallon is increasingly costly to produce.
We specifically focus on the most challenging setting of posted item prices\footnote{By virtue of posted pricing, our mechanisms are inherently incentive compatible.} in the face of an unknown series of buyers, with unknown and arbitrary combinatorial valuation functions, who arrive online.  That is, the seller (e.g., a supermarket) must assign prices to each of $n$ goods, then a buyer arrives with some arbitrary combinatorial valuation function and purchases the bundle maximizing her own quasilinear utility (valuation minus price).  After the buyer has made her purchase, the seller may adjust prices, then the next buyer arrives, and so on.  In this setting, the seller \emph{cannot} ask a buyer to submit her utility function, cannot run VCG, and cannot charge an admission fee to enter the store.  We consider two natural goals --  maximizing social welfare (the sum of buyers' valuations on bundles purchased, minus the costs incurred by the seller for obtaining these items)\footnote{Social welfare is a natural objective if we view the seller as a resource allocator within a company, and buyers as various units in the company needing resources.} and maximizing profit (the total amount paid by the buyers, minus the costs incurred by the seller).  Our main result is that using appropriate algorithms we can in fact perform nearly as well as in the much easier setting of digital goods for a wide range of cost curves.

A second scenario where our results are applicable is in the context of network routing with congestion. Specifically, we would like to maximize the sum of valuations of routed connections (each user has some pair of terminals and a valuation on receiving a connection) minus the congestion cost of routing them. The congestion cost can reflect either the energy required to support the traffic on the network or the cost of additional infrastructure needed to maintain the quality of service under increased load.~\citet{Andrews2010:Minimum} indicate that energy curves for processors exhibit dis-economies of scale i.e. energy expenditure is super-linear as a function of processor speed.  Such a scenario is captured by our model of increasing marginal cost, which for network routing would mean increasing marginal congestion costs.

We will sometimes refer to marginal cost to the seller of the $k^{th}$ copy of an item as the \emph{production cost} of the $k^{th}$ copy of that item.

\subsection{Our Results and Techniques}
We focus on two goals: maximizing social welfare, and maximizing profit.  Social welfare is the total valuation of the buyers for their bundles purchased, minus the cost to the seller of all items sold.   That is, it is the total utility of all players including the seller.  Note that because the production costs are not flat, even to maximize social welfare, one cannot simply sell items at their production costs; one must sell at a price higher than the production cost\footnote{See \lref[Appendix]{sec:at-cost-no-good} for an example.}. This is in order to ensure that items reach the buyers  who want them (approximately) most. The second goal is to maximize profit, i.e., the sum of prices charged for items sold minus their costs to the seller.

For a wide range of reasonable cost functions (linear, low-degree polynomial, logarithmic), we present a pricing scheme that achieves a social welfare within a {\em constant} factor of the optimal social welfare allocation minus a necessary additive loss. This holds for buyers with arbitrary combinatorial valuation functions.  Furthermore, the algorithm is quite `natural' and reasonable: we price the $k^{th}$ copy of any good at the production cost of the $2k^{th}$ copy\footnote{For illustrative examples showing why some closely related algorithms {\em fail}, see \lref[Appendix]{sec:egs}.}. This pricing scheme, that we call \emph{twice-the-index}, appears in \lref[Section]{sec:algo-twice-the-index}.

The Twice-the-index pricing scheme however fails to give good guarantees for all increasing cost functions. For instance, for the $0$-$\infty$ case, where the first few copies are available at zero cost and thereafter the copies have an extremely high production cost, buyer instances can be easily be created where twice-the-index fails to give any any `reasonable' guarantee (\lref[Appendix]{sec:twice-index-fails}). \cite{BGN03} propose a pricing scheme for the $0$-$\infty$ setting which achieves a logarithmic approximation to the social welfare in case the number of copies available at zero cost are logarithmically many. We build on their idea and apply it to an arbitrary increasing cost curve by breaking up the curve into contiguous chunks, each containing logarithmically many copies, and apply their pricing scheme separately for each chunk. This pricing scheme, presented in \lref[Section]{sec:algo-bgn}, gives roughly a logarithmic approximation to the optimal social welfare minus the production cost of logarithmically many initial copies.

While the Twice-the-index pricing scheme gives constant approximation guarantees for `nice' curves, the pricing scheme in \lref[Section]{sec:algo-bgn} gives a logarithmic approximation for arbitrary increasing curves. We would ideally want a single algorithm that can give us constant approximation guarantees for `nice' curves and logarithmic guarantees for arbitrary increasing curves. We achieve this for the case of \emph{convex} increasing curves. In \lref[Section]{sec:algo-smoothing}, we present a \emph{smoothing} pricing scheme that attains a constant approximation to the optimal social welfare for polynomial curves and a logarithmic approximation for arbitrary convex curves (plus some additive loss in both cases).

Interestingly, in order to prove the approximation guarantee for all of the presented social welfare maximizing schemes, we use a crucial result which we refer to as the \emph{Structural Lemma}. This result is stated and proved in \lref[Section]{sec:structure}. The result reduces the problem of proving the social welfare guarantee of a pricing scheme for buyers with arbitrary valuations to a case of proving that for \emph{every item}, the profit generated through sales of copies of the item is comparable to the area between the production curve of the item and a line parallel to $x$-axis and at a height equal to the prices of the lowest priced unsold copy of the item. Hence the Structural Lemma simplifies the analysis considerably since it allows the problem to be seen \emph{per item} even though the original problem is combinatorial.

Finally, in \lref[Section]{sec:profit}, we change our objective to maximizing the \emph{profit}, i.e., the sum of prices of goods sold minus the production cost of the goods. Here we give a randomized pricing scheme that takes as input any social welfare maximizing scheme (with approximation factor, say $\rho$) and a single-buyer profit maximizing pricing (with approximation factor say $\mu$), and combines them to get a profit maximization pricing scheme that achieve a ($\rho + \mu$) approximation to optimal profit for any sequence of buyers. In particular, we use the single-buyer profit maximization algorithm of \cite{BBM08} and combine it with the social-welfare pricing schemes mentioned above to get a logarithmic approximation to the optimal profit for arbitrary increasing curves. Our approach for combining a social welfare maximization pricing scheme with a single-buyer profit maximization algorithm is directly inspired by and builds upon a similar result presented in \cite{AAM03}. In fact, it extends their results to a more general setting with production costs and arbitrary valuations.


\subsection{Related work}
There is a huge body of literature on combinatorial auctions and pricing algorithms: we refer the reader to~\citep{BNisan, HartlineK} and the references therein---in particular, note~\citep{BGN03, lln06, DNS06,   Dob07, BriestKV05, LS05}. The setting of combinatorial auctions has been considered both in Bayesian (stochastic) settings, where the buyers' valuations are assumed to come from a known prior distribution, and non-Bayesian (adversarial) settings. Our work focuses on the non-Bayesian or adversarial setting. 

The algorithms of~\citet{BriestKV05} give truthful mechanisms that achieve constant approximations to social welfare for $\Omega(\log n)$ copies of each item (see also~\citep{APTT03}) in the \emph{offline} setting. For the \emph{online} setting, \citet{BGN03} give posted-price welfare-maximizing algorithms for combinatorial auctions in the limited supply setting---the approximation guarantees they give are logarithmic (when there are $\Omega(\log n)$ copies of each item) or worse (when there are fewer copies); their results are (nearly) tight for the online limited-supply setting. The smoothing algorithm presented in \lref[Section]{sec:algo-smoothing} generalizes the results of \citet{BGN03} to arbitrary increasing cost curves and not just $0$-$\infty$ costs (i.e. the limited supply case).  

The work of~\citet{AAM03} shows how to convert deterministic (or some special kind of randomized) online mechanisms for allocation problems into (randomized) posted-pricing schemes that achieve $(\rho + \log \vmax)$-fraction of the optimal profit possible, where the online algorithm is $\rho$-competitive for the allocation problem and $\vmax$ is the maximum valuation of any agent over the set of items. We extend their analysis to convert our social welfare maximizing algorithms to profit maximizing algorithms. The details of this conversion are given in \tfv{\lref[Section]{sec:profit}}.

\section{Model, Notation, and Definitions}
\label{sec:notation}

We consider the following setting.  A seller is selling a set $\items
=\{1, \ldots, n\}$ of $n$ items to a sequence $\buyers$ of $m$ buyers
who arrive one at a time.
%%This only matters for some results, so removing from here.
%(We assume we know $m$, this assumption can be removed at a
%further logarithmic loss.)
The seller can obtain (or produce) additional copies of each item but at increasing (or at least non-decreasing) production cost; specifically, let $\cost_i(k)$ denote the production cost to the seller for the $k$th copy of item $i$.  For each item $i$, let $\Cc_i(k)$ be the cumulative cost for the first $k$ copies---i.e., $\Cc_i(k) = \sum_{k' \leq k} \cost_i(k')$. Let $\cinv_i(p)$ be the number of copies of item $i$ available before the production cost exceeds $p$; in case $\cost_i(\cdot)$ is invertible, it follows that $\cinv_i(p)= \cost^{-1}_i(p)$.

Before each buyer arrives, the seller may mark up the costs to determine a sales price $\price_i$ for each item $i$. Every buyer $b$ has some (unknown to the seller) valuation function $v_b: 2^\items \to \R$ over possible bundles of items (we only require that $v_{b}(\phi)=0$ i.e. value on the empty bundle is zero), and purchases the utility-maximizing bundle for herself at the current prices.  That is, buyer $b$ purchases the set $S$ maximizing $v_b(S) - \sum_{i \in S} \price_i$.  After a buyer finishes purchasing her desired set, the seller may then readjust prices, and then the next buyer arrives, and so on.

For any particular sequence of buyers, let $\opt$ be the allocation that maximizes the social welfare. Clearly, the social welfare achieved under $\opt$, denoted by $\soc(\opt)$, is an upper bound on both the maximum social welfare and maximum profit achievable by any online algorithm.

For any algorithm $\alg$, $\soc(\alg)$ shall denote the social welfare attained through the algorithm. The algorithm shall determine a pricing scheme for the seller and $\price_i(k)$ shall denote the sales price charged for the $k^{th}$ copy of item $i \in \items$.  While this could in principle depend on other items sold, for all our algorithms it will depend only on $k$ and the cost-curve for the item.  $x_{i}$ shall denote the total number of copies of item $i$ sold by the algorithm, and $P^{f}_{i}$ shall denote the price of the first \emph{unsold} copy of item $i$---i.e., $P^{f}_{i} =  \price_i(x_{i}+1)$.

We shall denote the \emph{total production cost} suffered by the algorithm by $\Cc(\alg)$ and and the $\emph{revenue}$ made by $\Rev(\alg)$. $\prf_{i}$ shall denote the \emph{profit} made by the algorithm from the sales of item $i$. The total profit made by the algorithm is $\sum_{i \in \items}\prf_{i} = \Rev(\alg) - \Cc(\alg)$.

Since $x_{i}$ are the total number of copies sold by the algorithm $\alg$ for item $i$, therefore,  $\Cc(\alg)= \sum_{i\in \items} \sum_{k= 1}^{x_i} \cost_i(k)$, $\Rev(\alg)=\sum_{i\in \items} \sum_{k = 1}^{x_i} \price_i(k)$ and $\prf_{i}=\sum_{k = 1}^{x_i} \price_i(k) - \sum_{k =1}^{x_i} \cost_i(k)$.


The total valuation of buyers on their allocated bundles under $\alg$ is denoted by $V(\alg) = \sum_{b \in \buyers} v_b(\alg(b))$ where $\alg(b)$ denotes the set of items bought by buyer $b$ from the algorithm $\alg$.  The \emph{social welfare} made by the algorithm $\soc(\alg)$ is  $ V(\alg) - \Cc(\alg)$.

For $\opt$, the welfare-maximizing allocation, $\lambda_i$ denotes the number of copies of item $i$ allocated in $\opt$. $\Cc(\opt)$, $V(\opt)$ and $\soc(\opt)$ are defined analogously.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "marginv1"
%%% End:

